Cross-modal Embeddings for Video and Audio Retrieval

The increasing amount of online videos brings several opportunities for training self-supervised neural networks. The creation of large scale datasets of videos such as the YouTube-8M allows us to deal with this large amount of data in manageable way. In this work, we find new ways of exploiting this dataset by taking advantage of the multi-modal information it provides. By means of a neural network, we are able to create links between audio and visual documents, by projecting them into a common region of the feature space, obtaining joint audio-visual embeddings. These links are used to retrieve audio samples that fit well to a given silent video, and also to retrieve images that match a given a query audio. The results in terms of Recall@K obtained over a subset of YouTube-8M videos show the potential of this unsupervised approach for cross-modal feature learning. We train embeddings for both scales and assess their quality in a retrieval problem, formulated as using the feature extracted from one modality to retrieve the most similar videos based on the features computed in the other modality.

==> 3_dataset.tex <==
%%%% Dataset

This work is based on the 
On this project we take advantage of the recent creation of the YouTube-8M dataset \cite{youtube8m}. This dataset consist in more than 7 million videos labeled with an average of 3.4 labels. These videos are separated between the 4716 different classes. For organization proposes, these classes are grouped by categories and their distribution can be seen in Figure \ref{fig:entities}.

\begin{figure}[!hbt]
   	\includegraphics[width=\columnwidth]{figures/vertical-entities.png}
    \caption{Entities in the YouTube dataset grouped by category}
    \label{fig:entities}
\end{figure}

Each sample of the dataset does \emph{not} contain the raw video, but it is represented by previously extracted features, which are both visual and auditive (extracted and provided separately). 

The dataset provides \textit{video-level} features, which represent all the video using a single vector (one for audio and another for image), and thus does not maintain temporal information; and also provides \textit{frame-level} features, which consist on a single vector representing each second of audio, and a single vector representing each frame of the video, sampled at 1 frame per second. 

% Then, each sample provides information about:
% \begin{itemize}[noitemsep]
% \item Video ID, represented by the URL of the actual YouTube video. This is useful to retrieve the whole video when needed, instead of being limited to the provided features.
% \item List of labels.
% \item Frame-level audio features.
% \item Frame-level image features.
% \item Video-level audio features.
% \item Video-level image features.
% \end{itemize}

The main goal of this dataset is to provide enough data to reach state of the art results in video classification. Nevertheless, such a huge dataset also permits approaching other tasks related to videos and cross-modal tasks, such as the one we approach in this paper. For this work, and as a baseline, we only use the \textit{video-level} features. 

%The fact of not using the \textit{frame-level} features implies two main drawbacks. On the one hand, we lose temporal information related to the video, which is crucial for a correct match between image and audio. On the other hand, it prevents us from using a much bigger set of features for each video, restricting our system to work only with a small representation of it. We leave this to future work.

==> guideline.tex <==
\section{Introduction}
\label{sec:intro}

These guidelines include complete descriptions of the fonts, spacing, and related information for producing your proceedings manuscripts. Please follow them. If you have any questions, direct them to icme2018@gmail.com.

\subsection{Language}

All manuscripts must be in English.

\subsection{Paper length}

Papers should be no longer than 6 pages, including all text, figures, and references.

\subsection{Supplemental material}

Authors may optionally upload supplemental material. Typically, this material might include:
\begin{itemize}
  \item a short presentation summarizing the paper,
  \item videos of results that cannot be included in the main paper,
  \item screen recording of the running program
  \item anonymized related submissions to other conferences and journals, and
  \item appendices or technical reports containing extended proofs and mathematical derivations that are not essential for understanding of the paper.
\end{itemize}

Note that the contents of the supplemental material should be referred to appropriately in the paper and that reviewers are not obliged to look at it.

All supplemental material must be zipped into a single file. There is a 30MB limit on the size of this file.

\subsection{Dual submission}

By submitting a manuscript to ICME, the authors guarantee that it has not been previously published (or accepted for publication) in substantially similar form. Furthermore, no paper which contains significant overlap with the contributions of this paper either has been or will be submitted during the ICME 2018 review period to either a journal or a conference.

If there are papers that may appear to violate any of these conditions, then it is the authors' responsibility to (1) cite these papers (preserving anonymity as described in Section 2 of this example paper), (2) argue in the body of your paper why your ICME paper is nontrivially different from these concurrent submissions, and (3) include anonymized versions of those papers in the supplemental material.

\section{Blind Review}

Many authors misunderstand the concept of anonymizing for blind review. Blind review does not mean that one must remove citations to one's own work-in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work. That is all. (But see below for techreports)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith, it says that you are building on her work. If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]''and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our
   previous paper [1], and show it to be inferior to all
   previously known methods. Why the previous paper was
   accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}

An example of an excellent paper:

\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the
   paper of Smith [1], and show it to be inferior to
   all previously known methods.  Why the previous paper
   was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo
   filter, a fundamental contribution to human knowledge''.
   Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work. In such cases, include the anonymized parallel submission~\cite{Authors12} as additional material and cite it as

\begin{quote}
1. Authors. ``The frobnicatable foo filter'', ACM MM 2016 Submission ID 324, Supplied as additional material {\tt acmmm13.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report. For conference
submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a techreport for further details. Thus, you may say in
the body of the paper ``further details may be found in~\cite{Authors12b}''.  Then submit the techreport as additional material. Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool which is widely known to be restricted to a single institution.  For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the ICME audience would like to hear about your solution.  The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus.

You can handle this paper like any other.  Don't write ``We show how to improve our previous work [Anonymous, 1968].  This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''. That would be silly, and would immediately identify the authors. Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.  This
   system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] didn't
   handle case B properly.  Ours handles it by including
   a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo
   lunar lander, and went all the way to the moon, don't
   you know.  It displayed the following behaviours
   which show how well we solved cases A and B: ...
\end{quotation}

As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors. A reviewer might think it likely that the new paper was written by Zeus, but cannot make any decision based on that guess. He or she would have to be sure that no other authors could have been contracted to solve problem B.

FAQ: Are acknowledgements OK?  No. Please omit them in the review copy and leave them for the final copy.

\section{Formatting Your Paper}

All printed material, including text, illustrations, and charts, must be kept within a print area of 7 inches (178 mm) wide by 9 inches (229 mm) high. Do not write or print anything outside the print area. The top margin must be 1 inch (25 mm), except for the title page, and the left margin must be 0.75 inch (19 mm).  All text must be in a two-column format. Columns are to be 3.39 inches (86 mm) wide, with a 0.24 inch (6 mm) space between them. Text must be fully justified.

\section{Page Title Section}

The paper title (on the first page) should begin 1.38 inches (35 mm) from the top edge of the page, centered, completely capitalized, and in Times 14-point, boldface type.  The authors' name(s) and affiliation(s) appear below the title in capital and lower case letters.  Papers with multiple authors and affiliations may require two or more lines for this information.

\section{Type-Style and Fonts}

To achieve the best rendering both in the proceedings and from the CD-ROM, we strongly encourage you to use Times-Roman font. In addition, this will give the proceedings a more uniform look. Use a font that is no smaller than nine point type throughout the paper, including figure captions.

If you use the smallest point size, there should be no more than 3.2 lines/cm (8 lines/inch) vertically. This is a minimum spacing; 2.75 lines/cm (7 lines/inch) will make the paper much more readable. Larger type sizes require correspondingly larger vertical spacing. Please do not double-space your paper. True-Type 1 fonts are preferred.

The first paragraph in each section should not be indented, but all following paragraphs within the section should be indented as these paragraphs demonstrate.

\section{Major Headings}

Major headings, for example, ``1. Introduction'', should appear in all capital letters, bold face if possible, centered in the column, with one blank line before, and one blank line after. Use a period (``.'') after the heading number, not a colon.

\subsection{Subheadings}

Subheadings should appear in lower case (initial word capitalized) in boldface. They should start at the left margin on a separate line.

\subsubsection{Sub-subheadings}

Sub-subheadings, as in this paragraph, are discouraged. However, if you must use them, they should appear in lower case (initial word capitalized) and start at the left margin on a separate line, with paragraph text beginning on the following line.  They should be in italics.

\section{Page Numbering}

Please do {\bf not} paginate your paper. Page numbers, session numbers, and conference identification will be inserted when the paper is included in the proceedings.

% Below is an example of how to insert images. Delete the ``\vspace'' line,
% uncomment the preceding line ``\centerline...'' and replace ``imageX.ps''
% with a suitable PostScript file name.
% -------------------------------------------------------------------------
%
\begin{figure}[t]
\begin{minipage}[b]{1.0\linewidth}
  \centering
% \centerline{\epsfig{figure=image1.ps,width=8.5cm}}
  \vspace{1.5cm}
  \centerline{(a) Result 1}\medskip
\end{minipage}
%
\begin{minipage}[b]{.48\linewidth}
  \centering
% \centerline{\epsfig{figure=image3.ps,width=4.0cm}}
  \vspace{1.5cm}
  \centerline{(b) Results 2}\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.48\linewidth}
  \centering
% \centerline{\epsfig{figure=image4.ps,width=4.0cm}}
  \vspace{1.5cm}
  \centerline{(c) Result 3}\medskip
\end{minipage}
%
\caption{Example of placing a figure with experimental results.}
\label{fig:res}
\end{figure}

\section{Illustrations, Graphs, and Photographs}
\label{sec:illust}

Illustrations must appear within the designated margins. They may span the two columns. If possible, position illustrations at the top of columns, rather than in the middle or at the bottom. Caption and number every illustration. All halftone illustrations must be clear black and white prints.  Do not use any colors in illustrations.

Since there are many ways, often incompatible, of including images (e.g., with experimental results) in a \LaTeX document. Figure~\ref{fig:res} shows you an example of how to do this.

\section{Tables and Equations}

Tables and important equations must be centered in the column. Table~\ref{tab:cap} shows an example of a table while the equation
\begin{eqnarray}
y &=& ax^2+bx+c \nonumber \\
~ &=& (x+p)(x+q)
\end{eqnarray}
shows an example of an equation layout.

\begin{table}[t]
\begin{center}
\caption{Table caption} \label{tab:cap}
\begin{tabular}{|c|c|c|}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  Column One & Column Two & Column Three
  \\
  \hline
  Cell 1 & Cell 2 & Cell 3 \\
  Cell 4 & Cell 5 & Cell 6 \\
  \hline
\end{tabular}
\end{center}
\end{table}

Large tables or long equations may span across both columns. Any table or equation that takes up more than one column width must be positioned either at the top or at the bottom of the page.

\section{Footnotes}

Use footnotes sparingly (or not at all!) and place them at the bottom of the column on the page on which they are referenced. Use Times 9-point type, single-spaced. To help your readers, avoid using footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).

\section{Citations and References}

List and number all bibliographical references at the end of the paper. The references can be numbered in alphabetic order or in order of appearance in the document. When referring to them in the text, type the corresponding reference number in square brackets as shown at the end of this sentence~\cite{Morgan2005}. All citations must be adhered to IEEE format and style. Examples such as~\cite{Morgan2005},~\cite{cooley65} and~\cite{haykin02} are given in Section 12.

==> tables_results.tex <==
\begin{table*}
\begin{center}
\caption{From image to audio}
\label{table:results_subjective_ia}
\begin{tabular}{c|c c c}
	& Example1 & Example2 & Example3 \\
	\hline
	\multirow{3}{*}
		{Image} & 
		\multicolumn{1}{l}{{\includegraphics[width=0.3\textwidth]{figures/thumbnail_07.jpg}}} & 
		\multicolumn{1}{l}{{\includegraphics[width=0.3\textwidth]{figures/thumbnail_09.jpg}}} & 
		\multicolumn{1}{l}{{\includegraphics[width=0.3\textwidth]{figures/thumbnail_11.jpg}}} \\
		\cdashline{2-4} & 
		\multicolumn{1}{l}{\url{et4F0kzJe8k}} & 
		\multicolumn{1}{l}{\url{elv8Xt7u2uw}} & 
		\multicolumn{1}{l}{\url{a0CaARI3a4A}} \\
		\cdashline{2-4} & 
		\multicolumn{1}{l}{\specialcell{Korean comercial. \\Visual information: Korean letters, \\people and houses}} & 
		\multicolumn{1}{l}{\specialcell{Girl playing Gloomy Sunday on the \\piano. Visual information: hands and \\piano keys}} & 
		\multicolumn{1}{l}{\specialcell{Super Mario 64}} \\
                \cdashline{2-4} & 
		\multicolumn{1}{l}{\specialcell{23  Mobile phone \\29 Smartphone \\155 Camera \\566 Digital camera}} & 
		\multicolumn{1}{l}{\specialcell{36 Piano \\53 Strategy video game \\104 Pianist \\107 Motorcycling}} & 
		\multicolumn{1}{l}{\specialcell{0 Game \\2 Video game \\55 Video game console \\502 Sky \\973 Nintendo 64}} \\
	\hline
	\multirow{3}{*}
		{Audio} & 
		\multicolumn{1}{l}{{\includegraphics[width=0.3\textwidth]{figures/thumbnail_08.jpg}}} & 
		\multicolumn{1}{l}{{\includegraphics[width=0.3\textwidth]{figures/thumbnail_10.jpg}}} & 
		\multicolumn{1}{l}{{\includegraphics[width=0.3\textwidth]{figures/thumbnail_12.jpg}}}\\\cdashline{2-4} & 
		\multicolumn{1}{l}{\url{8l_uw8h0lPQ}} & 
		\multicolumn{1}{l}{\url{ayLROSsmUIs}} & 
		\multicolumn{1}{l}{\url{DHGgiM0Ym6Y}} \\
		\cdashline{2-4} & 
		\multicolumn{1}{l}{\specialcell{Korean comercial also. Audio \\information: Korean woman talking}} & 
		\multicolumn{1}{l}{\specialcell{Girl playing the piano. \\Audio information: piano sound}} & 
		\multicolumn{1}{l}{\specialcell{Videogame. The audio information is \\the music of the videogame, that at \\some point is the famous Mario one \\(which is always the same)}} \\
                \cdashline{2-4} & 
		\multicolumn{1}{l}{\specialcell{227 Water \\536 Glass}} & 
		\multicolumn{1}{l}{\specialcell{36 Piano \\53 Strategy video game \\107 Motorcycling \\265 Electronic keyboard}} & 
		\multicolumn{1}{l}{\specialcell{0 Game \\2 Video game \\55 Video game console}} \\
	\hline
\end{tabular}
\end{center}
\end{table*}

\begin{table*}
\begin{center}
\caption{From audio to image}
\label{table:results_subjective_ai}
\begin{tabular}{c|c c c}
	& Example1 & Example2 & Example3 \\
	\hline
	\multirow{3}{*}
		{Audio} & 
		\multicolumn{1}{l}{{\includegraphics[width=0.3\textwidth]{figures/thumbnail_01.jpg}}} & 
		\multicolumn{1}{l}{{\includegraphics[width=0.3\textwidth]{figures/thumbnail_03.jpg}}} & 
		\multicolumn{1}{l}{{\includegraphics[width=0.3\textwidth]{figures/thumbnail_05.jpg}}} \\
		\cdashline{2-4} & 
		\multicolumn{1}{l}{\url{15RmpSpN_rI}} & 
		\multicolumn{1}{l}{\url{HWmyh0DLF8k}} & 
		\multicolumn{1}{l}{\url{4rpfsxwfAw0}} \\
		\cdashline{2-4} & 
		\multicolumn{1}{l}{\specialcell{Russians fishing in a frozen river.\\Audio information: sound of water \\and russians talking}} & 
		\multicolumn{1}{l}{\specialcell{Embossing folder stamping with \\papertrey ink. Audio information: \\woman talking and sound of tools.}} & 
		\multicolumn{1}{l}{\specialcell{Kenny Chesney live concert recorded \\from the crowd}} \\
        \cdashline{2-4} & 
		\multicolumn{1}{l}{\specialcell{18 Outdoor recreation \\22 Nature \\42 Fishing \\84 Snow \\120 Winter \\262 Ice}} & 
		\multicolumn{1}{l}{\specialcell{242 Paper \\1063 Ink}} & 
		\multicolumn{1}{l}{\specialcell{3 Concert \\68 Lighting}} \\
	\hline
	\multirow{3}{*}
		{Image} & 
		\multicolumn{1}{l}{{\includegraphics[width=0.3\textwidth]{figures/thumbnail_02.jpg}}} & 
		\multicolumn{1}{l}{{\includegraphics[width=0.3\textwidth]{figures/thumbnail_04.jpg}}} & 
		\multicolumn{1}{l}{{\includegraphics[width=0.3\textwidth]{figures/thumbnail_06.jpg}}}\\\cdashline{2-4} & 
		\multicolumn{1}{l}{\url{ayD4L-JCxAY}} & 
		\multicolumn{1}{l}{\url{ayFc7SADE6k}} & 
		\multicolumn{1}{l}{\url{a0zIdifXB5Y}} \\
		\cdashline{2-4} & 
		\multicolumn{1}{l}{Russians swimming in a river} & 
		\multicolumn{1}{l}{\specialcell[l]{Recipe video of upside down apple \\cake}} & 
		\multicolumn{1}{l}{\specialcell{Jaguares live concert recorded from \\the crowd}} \\
        \cdashline{2-4} & 
		\multicolumn{1}{l}{\specialcell{18 Outdoor recreation \\147 River}} & 
		\multicolumn{1}{l}{\specialcell{12 Animal \\26 Cooking \\32 Recipe \\226 Dessert \\232 Cake \\236 Baking \\1319 Bangs (hair)}} & 
		\multicolumn{1}{l}{\specialcell{3 Concert}} \\
	\hline
\end{tabular}
\end{center}
\end{table*}







